Vcc: Scaling Transformers to 128K Tokens or More by Prioritizing Important Tokens

Transformers are central in modern natural language processing and computer vision applications. Despite recent works devoted to reducing the quadratic cost of such models (as a function of the sequence length), dealing with ultra long sequences (e.g., with more than 16K tokens) remains challenging. Applications such as answering questions based on a book or summarizing a scientific article are inefficient or infeasible. Here, we propose to significantly improve the efficiency of Transformers for ultra long sequences, by compressing the sequence into a much smaller representation at each layer. Specifically, by exploiting the fact that in many tasks, only a small subset of special tokens (we call VIP-tokens) are most relevant to the final prediction, we propose a VIP-token centric compression (VCC) scheme which selectively compresses the sequence based on their impact on approximating the representation of the VIP-tokens. Compared with competitive baselines, our algorithm is not only efficient (achieving more than $3\times$ efficiency gain compared to baselines on 4K and 16K lengths), but also offers competitive/better performance on a large number of tasks. Further, we show that our algorithm scales to 128K tokens (or more) while consistently offering accuracy improvement.

==> figures/components.tex <==

% \begin{figure}[!h]
% \centering
% % \vspace{-0.05in}
% \includegraphics[width=4in]{files/components.pdf}
% % \vspace{-0.2in}
% \caption{Visualization of $B_x^s$ for some scaling $s$ and translation $x$. The y axis for different plots are not the same. 
% }
% \label{fig:components}
% \vspace{-0.05in}
% \end{figure}

\begin{wrapfigure}{R}{0.5\textwidth}
\centering
\vspace{-0.15in}
\includegraphics[width=0.5\textwidth]{files/components.pdf}
\vspace{-0.15in}
\caption{Visualization of $B_x^s$ for some scaling $s$ and translation $x$. The y axis for different plots are not the same. 
}
\vspace{0.1in}
\label{fig:components}
\end{wrapfigure}

==> figures/segment_representation.tex <==
\begin{wrapfigure}{R}{0.42\textwidth}
\centering
% \vspace{-0.05in}
\includegraphics[width=0.42\textwidth]{files/refine_process.pdf}
\vspace{-0.2in}
\caption{
Illustration of multi-resolution compression. 
}
\label{fig:segment_rep}
\vspace{-0.1in}
\end{wrapfigure}

==> inserts/algo_no_cache.tex <==

% \setlength{\textfloatsep}{10pt}
% \begin{algorithm}[tb]
%    \caption{One layer computation}
%    \label{alg:compute_no_cache}
%    {\small
% \begin{algorithmic}
%     \STATE {\bfseries Input:} Input sequence $[Q; C]$
%     \STATE Compute $C^s$ for all $s$
%     \STATE Define method for retrieving $C^s_x$ from $C^s$
%     \STATE Use Algo. \ref{alg:construction_J} to construct $\mathcal{J}$
%     \STATE Construct $S_c, S_c C$ associated with $\mathcal{J}$
%     \STATE Compute $[\gamma(Q); \gamma(S_c C)]$ defined in \eqref{eq:breakdown_gamma}
%     \STATE Compute $[\hat{Q}'; \hat{C}'] = [\gamma(Q) + Q; S_c^\pinv \gamma(S_c C) + C]$
%     \STATE {\bfseries Output:} $[\hat{Q}'; \hat{C}']$
% \end{algorithmic}}
% \end{algorithm}

\begin{wrapfigure}{R}{0.5\textwidth}
    % \vspace{-0.25in}
    \begin{minipage}{0.5\textwidth}
    \begin{algorithm}[H]
   \caption{One layer computation}
   \label{alg:compute_no_cache}
   {\small
\begin{algorithmic}
    \STATE {\bfseries Input:} Input sequence 
    \STATE Construct $\mathcal{J}$ and the associated $\mS_c, \mS_c \mC$
    \STATE Compute $[\gamma(Q); \gamma(S_c C)]$ defined in \eqref{eq:breakdown_gamma}
    \STATE Compute $[\hat{Q}'; \hat{C}'] = [\gamma(Q) + Q; S_c^\pinv \gamma(S_c C) + C]$
    \STATE {\bfseries Output:} $[\hat{Q}'; \hat{C}']$
\end{algorithmic}}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

==> tables/cache.tex <==
\begin{table}[!htbp]
\vspace{-0.03in}
\begin{center}
\begin{scriptsize}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\multicolumn{8}{c}{$C_1^8$} \\
\midrule
\multicolumn{4}{c|}{$\Delta C_1^4$} & \multicolumn{4}{c}{$\Delta C_2^4$} \\
\midrule
\multicolumn{2}{c|}{$\Delta C_1^2$} & \multicolumn{2}{c|}{$\Delta C_2^2$} & \multicolumn{2}{c|}{$\Delta C_3^2$} & \multicolumn{2}{c}{$\Delta C_4^2$} \\
\midrule
$\Delta C_1^1$ & $\Delta C_2^1$ & $\Delta C_3^1$ & $\Delta C_4^1$ & $\Delta C_5^1$ & $\Delta C_6^1$ & $\Delta C_7^1$ & $\Delta C_8^1$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vspace{-0.12in}
\caption{Proposed tree structure cache
}
\label{tab:tree_cache}
\end{table}

==> tables/roberta-hotpotqa.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
Model & Size & Length & Runtime & EM & F1 \\
\midrule
RoBERTa & base & 512 & 19.9 & 35.1 & 44.9 \\
RoBERTa & base & 4096 & 422.3 & 62.2 & 76.1 \\
Big Bird & base & 4096 & 297.9 & 59.5 & 73.2 \\
Longformer & base & 4096 & 371.0 & 59.9 & 73.6 \\
Ours & base & 4096 & 114.6 & 60.9 & 74.6 \\
Ours* & base & 4096 & 114.6 & 61.4 & 75.0 \\
Ours* & large & 4096 & 285.8 & 66.7 & 80.0 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Dev set results for HotpotQA}
\label{tab:roberta-hotpotqa}
\end{table}

==> tables/roberta-loss_diff.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{ccc}
\toprule
Big Bird & Longformer & Ours \\
\midrule
$0.025$ & $0.017$ & $0.114$ \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vspace{-0.1in}
\caption{Log perplexity reduction from 50k steps to 250k steps}
\vspace{-0.05in}
\label{tab:roberta-pretrain-decrement}
\end{table}

==> tables/roberta-quality.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
Model & Size & Length & Runtime & Accuracy \\
\midrule
RoBERTa & base & 512 & 21.2 & 39.0 \\
RoBERTa & base & 4096 & 403.2 & 39.5 \\
Big Bird & base & 4096 & 307.0 & 38.5 \\
Longformer & base & 4096 & 368.0 & 27.9 \\
Ours & base & 4096 & 126.4 & 39.6 \\
Ours* & base & 4096 & 125.7 & 39.5 \\
Ours* & large & 4096 & 390.8 & 41.8 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Dev set results for QuALITY}
\label{tab:roberta-quality}
\end{table}

==> tables/roberta-wikihop.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
Model & Size & Length & Runtime & Accuracy \\
\midrule
RoBERTa & base & 512 & 19.6 & 67.6 \\
RoBERTa & base & 4096 & 414.1 & 75.2 \\
Big Bird & base & 4096 & 293.3 & 74.5 \\
Longformer & base & 4096 & 369.7 & 74.3 \\
Ours & base & 4096 & 108.0 & 75.9 \\
Ours* & base & 4096 & 126.7 & 76.4 \\
Ours* & large & 4096 & 394.3 & 79.6 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Dev set results for WikiHop}
\label{tab:roberta-quality}
\end{table}

==> tables/t5-arxiv.tex <==


\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccccccc}
\toprule
Method & Size & Length & Runtime (ms) & R-1 & R-2 & R-L  \\
\midrule
T5 & base & 512 & 58.97/20.52 & 28.9 & 8.6 & 25.6 \\
T5 & base & 4k & 645.36/549.11 & 44.4 & 18.4 & 39.9 \\
LongT5 & base & 16k & 1699.7/1370.36 & 48.5 & 21.7 & 43.7 \\
Sublinear & base & 16k & 672.78/392.13 & 48.5 & 21.4 & 43.9 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Dev set results for encoder-decoder models fintuning on Arxiv summarization. For runtime and memory efficiency, the left value is for the entire model, and the right value is for the encoder. }
\label{tab:sublinear_t5_arxiv}
\end{table}

==> tables/t5-hotpotqa.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lcccccccc}
\toprule
Method & Size & Length & Runtime (ms) & EM & F1 \\
\midrule
T5 & base & 512 & 26.3/20.5 & 34.1 & 44.4 \\
T5 & large & 512 & 84.1/67.0 & 36.9 & 47.8 \\
T5 & base & 4k & 594.3/550.6 & 64.2 & 77.5 \\
T5 & large & 4k & 1598.1/1598.1 & 68.0 & 81.3 \\
LongT5 & base & 4k & 271.3/233.7 & 62.3 & 75.7 \\
LED & base & 4k & 237.4/222.9 & 55.1 & 67.9 \\
Our & base & 4k & 155.4/127.4 & 64.5 & 77.7 \\
Our & large & 4k & 485.3/382.8 & 67.8 & 81.0 \\
Our & 3b & 4k & 1547.7/1197.1 & 70.2 & 83.2 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{WikiHop dev set results for encoder-decoder models}
\label{tab:sublinear_t5_arxiv}
\end{table}

==> tables/t5-qa.tex <==

\begin{table*}[!t]
\begin{center}
\begin{tiny}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccccccccccccc}
\toprule
Method & Size & \# Param & Length & \multicolumn{3}{c}{Qasper} & \multicolumn{3}{c}{QuALITY}  & \multicolumn{3}{c}{ContractNLI} & \multicolumn{3}{c}{NarrativeQA} \\
& & & & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} \\
\midrule
T5 & base & 223M & 512 & 31.8 / 20.5 & 10.8 & 16.4 & 29.3 / 20.5 & 33.6 & 47.3 & 24.0 / 20.5 & 73.5 & 73.5 & 26.8 / 20.5 & 2.0 & 11.3 \\
T5 & base & 223M & 4K & 608.2 / 551.7 & 13.2 & 29.1 & 596.3 / 551.2 & 34.7 & 47.4 & 579.0 / 551.6 & 86.8 & 86.8 & 593.4 / 547.6 & 3.8 & 13.3 \\
LongT5 & base & 248M & 16K & 1628.5 / 1421.3 & 16.2 & 33.4 & 1633.1 / 1439.7 & 35.8 & 48.5 & 1564.2 / 1462.5 & 85.1 & 85.1 & 1541.7 / 1370.2 & 5.2 & 15.6 \\
\rowcolor{Gray}
Ours & base & 223M & 16K & 538.3 / 391.6 & 16.0 & 30.8 & 557.1 / 419.2 & 36.5 & 48.7 & 484.2 / 393.1 & 87.0 & 87.0 & 518.2 / 394.4 & 5.0 & 15.8 \\
\midrule
T5 & large & 738M & 512 & 101.9 / 66.4 & 11.3 & 17.0 & 95.8 / 67.1 & 35.3 & 49.0 & 78.1 / 67.1 & 74.3 & 74.3 & - / - & - & - \\
T5 & large & 738M & 4K & - / - & - & - & 1760.5 / 1596.4 & 37.8 & 50.5 & 1702.4 / 1601.2 & 87.2 & 87.2 & - / - & - & - \\
\rowcolor{Gray}
Ours & large & 738M & 16K & 1679.6 / 1120.2 & 16.3 & 33.7 & 1753.6 / 1210.7 & 40.3 & 52.5 & 1440.6 / 1122.6 & 87.8 & 87.8 & 1551.7 / 1133.9 & 6.6 & 18.7 \\
\midrule
\rowcolor{Gray}
Ours & 3b & 3B & 16K & 6165.4 / 4637.3 & 19.0 & 38.2 & 6398.8 / 4962.7 & 45.2 & 56.0 & 5850.2 / 4665.9 & 88.5 & 88.5 & 6055.4 / 4659.4 & 8.2 & 21.2 \\
\bottomrule
\end{tabular}
\end{tiny}
\end{center}
\vspace{-0.1in}
\caption{Dev results for encoder-decoder models on Qasper, QuALITY, ContractNLI, and NarrativeQA. }
\label{tab:t5-3}
% \vspace{-0.07in}
\end{table*}

% \begin{table*}[!t]
% \begin{center}
% \begin{scriptsize}
% \setlength{\tabcolsep}{4.5pt}
% \begin{tabular}{lcccccccccccccc}
% \toprule
% Method & Size & Length & \multicolumn{3}{c}{Qasper} & \multicolumn{3}{c}{QuALITY}  & \multicolumn{3}{c}{ContractNLI} & \multicolumn{3}{c}{NarrativeQA} \\
% & & & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} \\
% \midrule
% T5 & base & 512 & 31.8 / 20.5 & 10.8 & 16.4 & 29.3 / 20.5 & 33.6 & 47.3 & 24.0 / 20.5 & 73.5 & 73.5 & 26.8 / 20.5 & 2.0 & 11.3 \\
% T5 & base & 4K & 608.2 / 551.7 & 13.2 & 29.1 & 596.3 / 551.2 & 34.7 & 47.4 & 579.0 / 551.6 & 86.8 & 86.8 & 593.4 / 547.6 & 3.8 & 13.3 \\
% LongT5 & base & 16K & 1628.5 / 1421.3 & 16.2 & 33.4 & 1633.1 / 1439.7 & 35.8 & 48.5 & 1564.2 / 1462.5 & 85.1 & 85.1 & 1541.7 / 1370.2 & 5.2 & 15.6 \\
% Ours & base & 16K & 538.3 / 391.6 & 16.0 & 30.8 & 557.1 / 419.2 & 36.5 & 48.7 & 484.2 / 393.1 & 87.0 & 87.0 & 518.2 / 394.4 & 5.0 & 15.8 \\
% \midrule
% T5 & large & 512 & 101.9 / 66.4 & 11.3 & 17.0 & 95.8 / 67.1 & 35.3 & 49.0 & 78.1 / 67.1 & 74.3 & 74.3 & - / - & - & - \\
% T5 & large & 4K & - / - & - & - & 1760.5 / 1596.4 & 37.8 & 50.5 & 1702.4 / 1601.2 & 87.2 & 87.2 & - / - & - & - \\
% Ours & large & 16K & 1679.6 / 1120.2 & 16.3 & 33.7 & 1753.6 / 1210.7 & 40.3 & 52.5 & 1440.6 / 1122.6 & 87.8 & 87.8 & 1551.7 / 1133.9 & 6.6 & 18.7 \\
% \midrule
% Ours & 3b & 16K & 6165.4 / 4637.3 & 19.0 & 38.2 & 6398.8 / 4962.7 & 45.2 & 56.0 & 5850.2 / 4665.9 & 88.5 & 88.5 & 6055.4 / 4659.4 & 8.2 & 21.2 \\
% \bottomrule
% \end{tabular}
% \end{scriptsize}
% \end{center}
% \vspace{-0.1in}
% \caption{Dev results for encoder-decoder models on Qasper, QuALITY, ContractNLI, and NarrativeQA. For runtime columns, the left value is for the entire model, and the right value is for the encoder. }
% \label{tab:t5-3}
% \vspace{-0.05in}
% \end{table*}

==> tables/t5-qasper.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lcccccccc}
\toprule
Method & Size & Length & Runtime (ms) & EM & F1 \\
\midrule
T5 & base & 512 & 25.7/20.5 & 66.7 & 69.1 \\
T5 & large & 512 & 83.5/67.0 & 69.1 & 71.4 \\
T5 & base & 4k & 594.3/553.7 & 76.2 & 78.1 \\
T5 & large & 4k & 1738.7/1601.0 & 79.1 & 80.7 \\
LongT5 & base & 4k & 270.7/233.9 & 72.7 & 74.8 \\
LED & base & 4k & 236.6/222.9 & 70.0 & 72.4 \\
Our & base & 4k & 181.7/148.1 & 76.7 & 78.4 \\
Our & large & 4k & 561.4/460.6 & 79.0 & 80.6 \\
Our & 3b & 4k & 1821.5/1441.2 & 80.8 & 82.3 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{WikiHop dev set results for encoder-decoder models}
\label{tab:sublinear_t5_arxiv}
\end{table}

==> tables/t5-sum.tex <==

\begin{table*}[!t]
\begin{center}
\begin{tiny}
\setlength{\tabcolsep}{1.3pt}
\begin{tabular}{lccccccccccccccccccc}
\toprule
Method & Size & \# Param & Length & \multicolumn{4}{c}{Arxiv} & \multicolumn{4}{c}{SummScreenFD}  & \multicolumn{4}{c}{GovReport} & \multicolumn{4}{c}{QMSum} \\
& & & & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} \\
\midrule
T5 & base & 223M & 512 & 59.0 / 20.5 & 28.9 & 8.6 & 25.6 & 59.1 / 20.5 & 27.0 & 4.8 & 23.5 & 59.1 / 20.5 & 40.5 & 14.8 & 38.2 & 43.5 / 20.5 & 30.2 & 8.0 & 26.5 \\
T5 & base & 223M & 4K & 645.4 / 549.1 & 44.4 & 18.4 & 39.9 & 647.9 / 551.1 & 31.6 & 6.8 & 27.6 & 648.3 / 551.5 & 54.0 & 25.2 & 51.4 & 620.2 / 551.5 & 31.1 & 8.2 & 27.4 \\
LongT5 & base & 248M & 16K & 1699.7 / 1370.4 & 48.5 & 21.7 & 43.7 & 1763.4 / 1427.8 & 33.1 & 7.3 & 28.5 & 1726.4 / 1387.7 & 55.8 & 27.9 & 53.2 & 1721.4 / 1450.7 & 35.7 & 11.7 & 31.4 \\
LED & base & 162M & 16K & 1055.8 / 923.6 & 47.8 & 20.6 & 43.2 & - / - & - & - & - & - / - & - & - & - & - / - & - & - & - \\
\rowcolor{Gray}
Ours & base & 223M & 16K & 672.8 / 392.1 & 48.5 & 21.4 & 43.9 & 670.5 / 390.9 & 33.1 & 7.3 & 28.6 & 674.0 / 391.6 & 55.2 & 27.1 & 52.6 & 623.1 / 396.5 & 31.8 & 8.8 & 27.9 \\
\midrule
T5 & large & 738M & 512 & 182.2 / 67.1 & 30.5 & 9.1 & 27.1 & 180.9 / 66.5 & 28.3 & 4.9 & 24.9 & 180.9 / 67.0 & 43.3 & 16.2 & 41.1 & 136.4 / 67.1 & 31.7 & 8.1 & 27.6 \\
T5 & large & 738M & 4K & 1901.5 / 1598.8 & 46.0 & 19.4 & 41.4 & - / - & - & - & - & - / - & - & - & - & - / - & - & - & - \\
\rowcolor{Gray}
Ours & large & 738M & 16K & 1959.1 / 1111.0 & 49.5 & 22.2 & 44.7 & 1957.1 / 1109.2 & 34.3 & 7.6 & 29.6 & 1955.5 / 1113.8 & 56.3 & 28.0 & 53.8 & 1816.4 / 1134.6 & 34.8 & 10.4 & 30.7 \\
\midrule
\rowcolor{Gray}
Ours & 3b & 3B & 16K & 7676.3 / 4642.2 & 49.8 & 22.4 & 45.0 & 7641.5 / 4631.3 & 34.7 & 7.8 & 30.1 & 7668.2 / 4642.7 & 56.9 & 28.5 & 54.3 & 7146.7 / 4655.6 & 35.7 & 10.9 & 31.1 \\
\bottomrule
\end{tabular}
\end{tiny}
\end{center}
\vspace{-0.1in}
\caption{Dev results for encoder-decoder models on Arxiv, SummScreenFD, GovReport, and QMSum. }
\label{tab:t5-2}
% \vspace{-0.17in}
\end{table*}

==> tables/t5-wikihop-hotpotqa-cnn_dailymail.tex <==

\begin{table*}[!t]
\begin{center}
\begin{tiny}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lccccccccccccccccc}
\toprule
Method & Size & \# Param & Length & \multicolumn{3}{c}{WikiHop} & \multicolumn{3}{c}{HotpotQA}  & \multicolumn{4}{c}{CNN/Dailymail} & \multicolumn{4}{c}{MediaSum} \\
& & & & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} &\tiny{R-L} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} \\
\midrule
T5 & base & 223M & 512 & 25.7 / 20.5 & 66.7 & 69.1 & 26.3 / 20.5 & 34.1 & 44.4 & 40.0 / 20.5 & 43.3 & 20.5 & 40.4 & 39.9 / 20.5 & 30.7 & 14.5 & 28.1 \\
T5 & base & 223M & 4K & 594.3 / 553.7 & 76.2 & 78.1 & 594.3 / 550.6 & 64.2 & 77.5 & 614.4 / 549.4 & 43.8 & 20.9 & 41.0 & 613.5 / 552.9 & 34.9 & 17.2 & 31.9 \\
LongT5 & base & 248M & 4K & 270.7 / 233.9 & 72.7 & 74.8 & 271.3 / 233.7 & 62.3 & 75.7 & 291.6 / 234.9 & 43.3 & 20.6 & 40.5 & 287.3 / 229.5 & 34.9 & 17.3 & 32.0 \\
LED & base & 162M & 4K & 236.6 / 222.9 & 70.0 & 72.4 & 237.4 / 222.9 & 55.1 & 67.9 & 249.4 / 221.8 & 43.3 & 20.0 & 40.5 & - / - & - & - & - \\
\rowcolor{Gray}
Ours & base & 223M & 4K & 181.7 / 148.1 & 76.7 & 78.4 & 155.4 / 127.4 & 64.5 & 77.7 & 195.8 / 139.9 & 43.6 & 20.7 & 40.7 & 196.7 / 140.2 & 34.8 & 17.3 & 31.9 \\
\midrule
T5 & large & 738M & 512 & 83.5 / 67.0 & 69.1 & 71.4 & 84.1 / 67.0 & 36.9 & 47.8 & 124.6 / 67.0 & 43.8 & 20.7 & 40.9 & 124.5 / 67.0 & 31.9 & 15.5 & 29.1 \\
T5 & large & 738M & 4K & 1738.7 / 1601.0 & 79.1 & 80.7 & 1598.1 / 1598.1 & 68.0 & 81.3 & 1824.8 / 1600.4 & 44.3 & 21.0 & 41.4 & - / - & - & - & - \\
\rowcolor{Gray}
Ours & large & 738M & 4K & 561.4 / 460.6 & 79.0 & 80.6 & 485.3 / 382.8 & 67.8 & 81.0 & 608.1 / 433.8 & 44.4 & 21.4 & 41.5 & 609.7 / 434.4 & 35.8 & 18.2 & 32.8 \\
\midrule
\rowcolor{Gray}
Ours & 3b & 3B & 4K & 1821.5 / 1441.2 & 80.8 & 82.3 & 1547.7 / 1197.1 & 70.2 & 83.2 & 1930.7 / 1364.8 & 44.8 & 21.5 & 41.9 & 1930.7 / 1364.8 & 36.3 & 18.5 & 33.3 \\
\bottomrule
\end{tabular}
\end{tiny}
\end{center}
\vspace{-0.1in}
\caption{Dev set results for encoder-decoder models finetuning on WikiHop, HotpotQA, CNN/Dailymail, and MediaSum. For runtime columns, the left value is for the entire model, and the right value is for the encoder. }
\label{tab:t5-1}
% \vspace{-0.07in}
\end{table*}

% \begin{table*}[!t]
% \begin{center}
% \begin{scriptsize}
% \setlength{\tabcolsep}{3.5pt}
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% Method & Size & Length & \multicolumn{3}{c}{WikiHop} & \multicolumn{3}{c}{HotpotQA}  & \multicolumn{4}{c}{CNN/Dailymail} & \multicolumn{4}{c}{MediaSum} \\
% & & & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{EM} & \tiny{F1} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} &\tiny{R-L} & \tiny{Runtime} & \tiny{R-1} & \tiny{R-2} & \tiny{R-L} \\
% \midrule
% T5 & base & 512 & 25.7 / 20.5 & 66.7 & 69.1 & 26.3 / 20.5 & 34.1 & 44.4 & 40.0 / 20.5 & 43.3 & 20.5 & 40.4 & 39.9 / 20.5 & 30.7 & 14.5 & 28.1 \\
% T5 & base & 4K & 594.3 / 553.7 & 76.2 & 78.1 & 594.3 / 550.6 & 64.2 & 77.5 & 614.4 / 549.4 & 43.8 & 20.9 & 41.0 & 613.5 / 552.9 & 34.9 & 17.2 & 31.9 \\
% LongT5 & base & 4K & 270.7 / 233.9 & 72.7 & 74.8 & 271.3 / 233.7 & 62.3 & 75.7 & 291.6 / 234.9 & 43.3 & 20.6 & 40.5 & 287.3 / 229.5 & 34.9 & 17.3 & 32.0 \\
% LED & base & 4K & 236.6 / 222.9 & 70.0 & 72.4 & 237.4 / 222.9 & 55.1 & 67.9 & 249.4 / 221.8 & 43.3 & 20.0 & 40.5 & - / - & - & - & - \\
% Ours & base & 4K & 181.7 / 148.1 & 76.7 & 78.4 & 155.4 / 127.4 & 64.5 & 77.7 & 195.8 / 139.9 & 43.6 & 20.7 & 40.7 & 196.7 / 140.2 & 34.8 & 17.3 & 31.9 \\
% \midrule
% T5 & large & 512 & 83.5 / 67.0 & 69.1 & 71.4 & 84.1 / 67.0 & 36.9 & 47.8 & 124.6 / 67.0 & 43.8 & 20.7 & 40.9 & 124.5 / 67.0 & 31.9 & 15.5 & 29.1 \\
% T5 & large & 4K & 1738.7 / 1601.0 & 79.1 & 80.7 & 1598.1 / 1598.1 & 68.0 & 81.3 & 1824.8 / 1600.4 & 44.3 & 21.0 & 41.4 & - / - & - & - & - \\
% Ours & large & 4K & 561.4 / 460.6 & 79.0 & 80.6 & 485.3 / 382.8 & 67.8 & 81.0 & 608.1 / 433.8 & 44.4 & 21.4 & 41.5 & 609.7 / 434.4 & 35.8 & 18.2 & 32.8 \\
% \midrule
% Ours & 3b & 4K & 1821.5 / 1441.2 & 80.8 & 82.3 & 1547.7 / 1197.1 & 70.2 & 83.2 & 1930.7 / 1364.8 & 44.8 & 21.5 & 41.9 & 1930.7 / 1364.8 & 36.3 & 18.5 & 33.3 \\
% \bottomrule
% \end{tabular}
% \end{scriptsize}
% \end{center}
% \vspace{-0.1in}
% \caption{Dev set results for encoder-decoder models finetuning on WikiHop, HotpotQA, CNN/Dailymail, and MediaSum. For runtime columns, the left value is for the entire model, and the right value is for the encoder. }
% \label{tab:t5-1}
% \vspace{-0.05in}
% \end{table*}

==> tables/t5-wikihop.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lcccccccc}
\toprule
Method & Size & Length & Runtime (ms) & EM & F1 \\
\midrule
T5 & base & 512 & 25.7/20.5 & 66.7 & 69.1 \\
T5 & large & 512 & 83.5/67.0 & 69.1 & 71.4 \\
T5 & base & 4k & 594.3/553.7 & 76.2 & 78.1 \\
T5 & large & 4k & 1738.7/1601.0 & 79.1 & 80.7 \\
LongT5 & base & 4k & 270.7/233.9 & 72.7 & 74.8 \\
LED & base & 4k & 236.6/222.9 & 70.0 & 72.4 \\
Our & base & 4k & 181.7/148.1 & 76.7 & 78.4 \\
Our & large & 4k & 561.4/460.6 & 79.0 & 80.6 \\
Our & 3b & 4k & 1821.5/1441.2 & 80.8 & 82.3 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{WikiHop dev set results for encoder-decoder models}
\label{tab:sublinear_t5_arxiv}
\end{table}

==> tables/t5.tex <==

\input{tables/t5-wikihop-hotpotqa-cnn_dailymail.tex}
\input{tables/t5-qa.tex}
\input{tables/t5-sum.tex}
\input{tables/t5-multi_news.tex}
\input{tables/t5-narrative_qa.tex}
